Practical gates by Majorana fermion motion

Quantum error correction protocols protect against local errors by storing logical information non-locally. This poses a challenge: how to design efficient logical gates on the non-local ``hidden'' logical information, and how to implement these gates using the local physical operations. We develop a general description of planar Pauli stabilizer codes and protocols for logical operations in terms of point-like particles called Majorana fermions. Information is stored in the pairwise fermion parities of spatially separated Majorana fermions. The description in terms of Majorana fermions captures not only large distance asymptotics, but also all scales down to the lattice constants. We exploit this locality to densely pack logical information in spacetime. The simplest application is to a static case: dense memory. More importantly, we implement fault-tolerant Majorana motion and leverage this primitive to design braiding-based logical gates. This approach reduces space overhead of logical operations resulting in an improved logical error rate given fixed number of physical qubits. We illustrate a practical use of our approach by designing and benchmarking of 2-qubit Clifford gates. We find numerically that our protocol outperforms lattice surgery in this setting for near-term error rates and realistic device constraints. More generally, introduction of compact motion of Majorana fermions as an efficient computational primitive opens a promising new route for the design of low overhead error correction protocols.

==> figures/lib/color-palette.tex <==
\definecolor{majoranavertex}{RGB}{148,17,0}
% Blue MJD
% \definecolor{majoranadiamondedge}{RGB}{47,82,143}
\definecolor{majoranadiamondedge}{HSB}{0,0,110}
\definecolor{majoranavertexlabel}{RGB}{255,255,255}
\definecolor{pscanyoncolor}{RGB}{148,55,255}
\definecolor{wilsonline}{RGB}{16,110,186}
\definecolor{wilsonlinealt}{RGB}{237,65,67}
\definecolor{tau1link}{RGB}{37, 95, 220}
\definecolor{tau2link}{RGB}{249, 195, 0}
\definecolor{tau3link}{RGB}{151, 209, 29}
\definecolor{psclink}{RGB}{43,43,43}
\definecolor{flippingmajorana}{RGB}{255,143,0}
\definecolor{thooftline}{RGB}{163,178,45}
\definecolor{stabilizerflux}{RGB}{178,161,199}

==> figures/lib/old-mm-na-preamble.tex <==
\RequirePackage[rgb]{xcolor}
% bugfix for HSB
\selectcolormodel{natural}
\RequirePackage{ninecolors}
\selectcolormodel{rgb}

\RequirePackage{tikz}
% \RequirePackage{\figdir/fade-no-fill}

\RequirePackage{tabularray}
\UseTblrLibrary{booktabs}

\RequirePackage{expl3}
\RequirePackage{xparse}
\RequirePackage{etoolbox}

\usetikzlibrary{calc,fadings,decorations.markings,%
positioning,decorations.pathmorphing,shapes.geometric,shadows,%
fit,%
arrows.meta,%
knots,%
3d,%
backgrounds,%
intersections}

\usetikzlibrary{overlay-beamer-styles}

% provides semifill
\makeatletter
\tikzset{
  prefix after node/.style={
    prefix after command={\pgfextra{#1}}
  },
  /semifill/ang/.store in=\semi@ang,
  /semifill/ang=0,
  semifill/.style={
    circle, draw,
    prefix after node={
      \typeout{aaa \semi@ang}
      \let\nodename\tikz@last@fig@name
      \fill[/semifill/.cd, /semifill/.search also={/tikz}, #1]
      let \p1 = (\nodename.north), \p2 = (\nodename.center) in
      let \n1 = {\y1 - \y2} in
      (\nodename.\semi@ang) arc [radius=\n1, start angle=\semi@ang, delta angle=180];
    },
  }
}

\pgfmathdeclarefunction{memberQ}{2}{%
  \begingroup%
    \edef\pgfutil@tmpb{0}%
    \edef\pgfutil@tmpa{#2}%
    \expandafter\pgfmath@member@i\pgfutil@firstofone#1\pgfmath@token@stop
    \edef\pgfmathresult{\pgfutil@tmpb}%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup}
\def\pgfmath@member@i#1{%
    \ifx\pgfmath@token@stop#1%
    \else
      \ifnum#1=\pgfutil@tmpa\relax%
      \gdef\pgfutil@tmpb{1}%
      %\typeout{#1=\pgfutil@tmpa}
      \fi%
      \expandafter\pgfmath@member@i
    \fi}
\makeatother

\pgfset{
  foreach/parallel foreach/.style args={#1in#2via#3}{evaluate=#3 as #1 using {{#2}[#3-1]}},
}


\def\drawmjverts#1{%
\foreach \carddir in {north,south,east,west} {
\node[majorana vertex] (#1-mj-\carddir) at (#1.\carddir) {};
}
}

\def\drawlabelledmjverts#1#2{%
\foreach \carddir [count=\count] in {north,south,east,west} {
\node[majorana labelled vertex] (#1-mj-\carddir) at (#1.\carddir) {\(\alpha_{#2\count}\)};
}
}

\def\drawonlykarrows#1#2{%
\begin{scope}[every path/.style={majorana diamond edge}]
\def\basemj{#1}
\def\kastpairs{#2}
\foreach \pstart/\pend in \kastpairs {
\draw[kasteleyn arrow] (\basemj-\pstart) -- (\basemj-\pend);
}
\end{scope}}

\def\drawkarrows#1#2{%
\drawmjverts{#1}
\drawonlykarrows{#1-mj}{#2}}

\def\drawdiamondkasteleyn#1#2{%
\ifcase#2\relax
\drawonlykarrows{#1-mj}{east/south,north/west,east/north,west/south}
\or
\drawonlykarrows{#1-mj}{south/east,west/north,east/north,west/south}
\or
\drawonlykarrows{#1-mj}{south/east,west/north,north/east,south/west}
\or
\drawonlykarrows{#1-mj}{east/south,north/west,north/east,south/west}
\or
\drawonlykarrows{#1-mj}{south/east,north/west,north/east,west/south}
\or
\drawonlykarrows{#1-mj}{south/east,north/west,east/north,south/west}
\or
\drawonlykarrows{#1-mj}{east/south,west/north,north/east,west/south}
\or
\drawonlykarrows{#1-mj}{east/south,west/north,east/north,south/west}
\fi}

\def\drawcoloreddiamondkasteleyn#1#2{%
\ifcase#2\relax
\begin{scope}[majorana diamond edge/.append style={tau1link}]
\drawonlykarrows{#1-mj}{east/south,north/west}
\end{scope}
\begin{scope}[majorana diamond edge/.append style={tau2link}]
\drawonlykarrows{#1-mj}{east/north,west/south}
\end{scope}
\or
\begin{scope}[majorana diamond edge/.append style={tau1link}]
\drawonlykarrows{#1-mj}{south/east,west/north}
\end{scope}
\begin{scope}[majorana diamond edge/.append style={tau2link}]
\drawonlykarrows{#1-mj}{east/north,west/south}
\end{scope}
\or
\begin{scope}[majorana diamond edge/.append style={tau1link}]
\drawonlykarrows{#1-mj}{south/east,west/north}
\end{scope}
\begin{scope}[majorana diamond edge/.append style={tau2link}]
\drawonlykarrows{#1-mj}{north/east,south/west}
\end{scope}
\or
\begin{scope}[majorana diamond edge/.append style={tau1link}]
\drawonlykarrows{#1-mj}{east/south,north/west}
\end{scope}
\begin{scope}[majorana diamond edge/.append style={tau2link}]
\drawonlykarrows{#1-mj}{north/east,south/west}
\end{scope}
\or
\begin{scope}[majorana diamond edge/.append style={tau1link}]
\drawonlykarrows{#1-mj}{south/east,north/west}
\end{scope}
\begin{scope}[majorana diamond edge/.append style={tau2link}]
\drawonlykarrows{#1-mj}{north/east,west/south}
\end{scope}
\or
\begin{scope}[majorana diamond edge/.append style={tau1link}]
\drawonlykarrows{#1-mj}{south/east,north/west}
\end{scope}
\begin{scope}[majorana diamond edge/.append style={tau2link}]
\drawonlykarrows{#1-mj}{east/north,south/west}
\end{scope}
\or
\begin{scope}[majorana diamond edge/.append style={tau1link}]
\drawonlykarrows{#1-mj}{east/south,west/north}
\end{scope}
\begin{scope}[majorana diamond edge/.append style={tau2link}]
\drawonlykarrows{#1-mj}{north/east,west/south}
\end{scope}
\or
\begin{scope}[majorana diamond edge/.append style={tau1link}]
\drawonlykarrows{#1-mj}{east/south,west/north}
\end{scope}
\begin{scope}[majorana diamond edge/.append style={tau2link}]
\drawonlykarrows{#1-mj}{east/north,south/west}
\end{scope}
\fi}

\def\drawmajoranadiamond#1#2{%
\drawmjverts{#1}
\drawdiamondkasteleyn{#1}{#2}}

\def\drawcoloredmajoranadiamond#1#2{%
\drawmjverts{#1}
\drawcoloreddiamondkasteleyn{#1}{#2}}

\def\drawlabelledmajoranadiamond#1#2#3{%
\drawlabelledmjverts{#1}{#3}
\drawdiamondkasteleyn{#1}{#2}}

\newcommand{\inputtosavebox}[2]{%
\expandafter\newsavebox\csname #1box\endcsname
\expandafter\savebox\csname #1box\endcsname{\input{#2}}
\expandafter\newcommand\csname #1\endcsname[1][]{\node[##1] {\expandafter\usebox\csname #1box\endcsname}}
}

\newcommand{\setfigdraftgeom}[1][9in]{%
\RequirePackage[margin=0pt,paperwidth=6.5in,paperheight=#1]{geometry}
\pagestyle{empty}%
}

\newcommand{\figdraft}[1][9in]{%
\providebool{standalone}
\ifstandalone
\else
\setfigdraftgeom[#1]\AtBeginDocument{\noindent}
\fi%
}

% graph handling

\ExplSyntaxOn
\seq_new:N \g_subgraphnodes
\NewDocumentCommand{\setsubgraph}{m}{
\seq_gset_split:NnV \g_subgraphnodes {,} {#1}}
\NewDocumentCommand{\ifsubgraphnode}{m m m}{
    \seq_if_empty:NTF \g_subgraphnodes {#2} {\seq_if_in:NVTF \g_subgraphnodes {#1} {#2} {#3}}}
\NewDocumentCommand{\whensubgraphnode}{m m}{\ifsubgraphnode{#1}{#2}{}}
\ExplSyntaxOff
\newcommand{\setupgraph}{%
\pkginclude{.}{example-psc-graph-spec}
\pkginclude{.}{example-majorana-graph-spec}}

\newcommand{\drawcoloreddiamond}[3][]{
\node[majorana diamond guide,#1] (#2) {};
\ifnum#3=0
\def\nwcolor{tau1link}
\def\swcolor{tau2link}
\else
\def\swcolor{tau1link}
\def\nwcolor{tau2link}
\fi
\begin{scope}[every path/.style={majorana diamond edge,line cap=round}]
\draw[\nwcolor] (#2.west) -- (#2.north);
\draw[\nwcolor] (#2.south) -- (#2.east);
\draw[\swcolor] (#2.west) -- (#2.south);
\draw[\swcolor] (#2.north) -- (#2.east);
\end{scope}
}

% Wilson lines
\ExplSyntaxOn
\seq_new:N \g_wilsonverts
\seq_new:N \g_wilsonlinetypes
\cs_new:Nn \wilson_setpartsmjvs:n {
  \seq_clear:N \g_wilsonverts
  \seq_clear:N \g_wilsonlinetypes
  \int_zero:N \l_tmpa_int
  \seq_set_split:Nnn \l_tmpa_seq {~} {#1}
  \seq_map_inline:Nn \l_tmpa_seq
  {
    \int_if_even:nTF \l_tmpa_int
    {\seq_put_right:Nn \g_wilsonverts {(##1.center)}}
    {\seq_put_right:Nn \g_wilsonlinetypes {##1}}
    \int_incr:N \l_tmpa_int
  }
}
\cs_new:Nn \wilson_setparts:n {
\seq_clear:N \g_wilsonverts
\seq_clear:N \g_wilsonlinetypes
\int_zero:N \l_tmpa_int
\seq_set_split:Nnn \l_tmpa_seq {~} {#1}
\seq_map_inline:Nn \l_tmpa_seq
{
\int_if_even:nTF \l_tmpa_int
{\seq_put_right:Nn \g_wilsonverts {##1}}
{\seq_put_right:Nn \g_wilsonlinetypes {##1}}
\int_incr:N \l_tmpa_int
}
}
\NewDocumentCommand{\setwilsonlinemjvs}{m}{
  \wilson_setpartsmjvs:n {#1}
}
\NewDocumentCommand{\setwilsonline}{m}{
\wilson_setparts:n {#1}
}
\NewDocumentCommand{\drawwilsonline}{O{}}{
  \seq_pop_left:NN \g_wilsonverts \l_vert
  \seq_map_inline:Nn \g_wilsonlinetypes {
    \seq_pop_left:NN \g_wilsonverts \l_vertb
    \xdef\etemp{\noexpand\draw[wilson~line,#1] \l_vert~##1~\l_vertb;}
    \etemp
    \xdef\l_vert{\l_vertb}
  }
}
\ExplSyntaxOff

% colors
\pkginclude{color-palette}

\tikzset{shadowed/.style={preaction={transform canvas={shift={(0.07,-.05)}},draw=gray,very thick,opacity=0.7}}}

\tikzset{figure-label/.style={font=\fontsize{9}{9}\selectfont}}
\tikzset{figure-sublabel/.style={font=\fontsize{7}{7}\selectfont}}

\tikzset{%
psc-spin-node/.style={draw,circle,minimum size=.4cm},
psc-d3v-spin-node/.style={psc-spin-node,draw=pscanyoncolor,semifill={pscanyoncolor,ang=180}},
psc-d2v-spin-node/.style={psc-spin-node,draw=pscanyoncolor,fill=pscanyoncolor},
psc-edge/.style={draw,line width=4pt,psclink},
psc-unconnected-edge/.style={psc-edge},
majorana vertex/.style={draw,fill,circle,inner sep=0pt,minimum size=.37cm,majoranavertex},
majorana labelled vertex/.style={majorana vertex,text=majoranavertexlabel},
majorana equality rectangle/.style={draw, rectangle, minimum width=1.8cm, minimum height=.55cm, rounded corners, orange, line width=2pt},
majorana blowup arrow/.style={->,opacity=0.7},
karrow/.tip={Stealth[length=.3cm,width=.4cm]},
kasteleyn arrow/.style={decoration={markings, mark=at position 0.5 with {\arrow[xshift=4pt]{karrow}}},
postaction={decorate}},
rev kasteleyn arrow/.style={decoration={markings, mark=at position 0.5 with {\arrow[xshift=-4pt,rotate=180]{karrow}}},
postaction={decorate}},
majorana diamond edge/.style={line width=2pt, draw=majoranadiamondedge},
majorana diamond guide/.style={minimum size=1.5cm,shape=diamond,inner sep=0pt},
labelled majorana diamond guide/.style={majorana diamond guide, minimum size=2.3cm},
majorana diamond/.style={majorana diamond guide, majorana diamond edge},
wilson line amplitude/.initial=2,
wilson line segment length/.initial=7,
wilson line decoration/.style={decoration={snake,
amplitude=\pgfkeysvalueof{/tikz/wilson line amplitude},
segment length=\pgfkeysvalueof{/tikz/wilson line segment length}},
decorate},
wilson line/.style={line width=1.7pt, wilsonline, wilson line decoration, line cap=round},
wilson arrow/.style={dart, inner sep=2,sloped,fill=wilsonline},
particle node/.style={circle,fill=majoranavertex,draw=majoranavertex, minimum size=0.2cm},
particle world line/.style={majoranavertex, line width=3pt},
virtual boundary/.style={dashed, draw=black,fill=white,opacity=0.7},
stabilizer flux/.style={fill=stabilizerflux,opacity=0.3},
thooft line/.style={line width=4pt, draw=thooftline},
thooft arrow/.style={wilson arrow,midway,fill=thooftline,draw=thooftline,minimum size=.3cm},
thooft majorana hl/.style={circle, flippingmajorana, minimum size=.4cm,draw, line width=2pt},
thooft wilson line/.style={lattice wilson line, circle, flippingmajorana, minimum size=.4cm,draw, line width=2pt},
transition arrow/.style={line width=5pt,-{Triangle[width=10pt,length=7pt]},gray},
braid line/.style={black, line width=2pt},
% real fonts/.style={every node/.append style={font=\fontsize{10}{10}\selectfont}},
real fonts/.style={},
time arrow/.style={thick, ->},
}

\tikzset{particle/.style={majorana vertex},
  free region/.style={fill=black, fill opacity=0.1, draw},
  worldline/.style={particle world line},
  physical-qubit/.style={circle, minimum size=.2cm, inner sep=0pt, shading=ball, ball color=blue},
  psc-spin-node/.style={physical-qubit},
  tau3link/.style={green!50!black}}

\pkginclude{surface-code-utils}


==> figures/lib/surface-code-utils.tex <==
\ExplSyntaxOn
\seq_new:N \g_excludededges
\NewDocumentCommand{\resetexcludeedges}{}{%
  \seq_clear:N \g_excludededges
}
\NewDocumentCommand{\excludeedges}{m}{%
  \seq_set_split:NnV \l_tmpexcludededges {,} {#1}
  \seq_concat:NNN \g_excludededges \g_excludededges \l_tmpexcludededges
}
\NewDocumentCommand{\ifsubedge}{m m m}{%
    \seq_if_empty:NTF \g_excludededges {#2} {\seq_if_in:NVTF \g_excludededges {#1} {#3} {#2}}
  }
\NewDocumentCommand{\whensubedge}{m m}{\ifsubedge{#1}{#2}{}}
\ExplSyntaxOff
\newcounter{edgecounter}
\NewDocumentCommand{\doedge}{m}{%
  \edef\tmpcounter{\theedgecounter}
  \whensubedge{\tmpcounter}{#1}
  \stepcounter{edgecounter}
}
\NewDocumentCommand{\drawsubedge}{O{psc-edge} m}{%
  \doedge{\draw[#1] #2;}
}

% surface code
% pass in nx, ny
\NewDocumentCommand{\drawscqubitsgen}{O{(0,0)} O{1.2} O{4} O{4} m}{
  \begin{scope}[scale=#2,shift={#1}]
    \foreach \x in {0,...,#3} {
      \foreach \y in {0,...,#4} {
        \drawcoloreddiamond[at={(\x,\y)}]{#5-\x-\y}{0}
      }
    }
    \pgfmathtruncatemacro{\xmo}{#3-1}
    \pgfmathtruncatemacro{\ymo}{#4-1}
    \foreach \x in {0,...,\xmo} {
      \foreach \y in {0,...,\ymo} {
        \pgfmathsetmacro{\midx}{\x+.5}
        \pgfmathsetmacro{\midy}{\y+.5}
        \coordinate (bulk-pl-\x-\y) at (\midx,\midy);
      }
    }
  \end{scope}
}

\NewDocumentCommand{\drawscqubits}{O{(0,0)} O{1.2} m}{
  \begin{scope}[scale=#2,shift={#1}]
    \foreach \x in {0,...,4} {
      \foreach \y in {0,...,4} {
        \drawcoloreddiamond[at={(\x,\y)}]{#3-\x-\y}{0}
      }
    }
    \foreach \x in {0,...,3} {
      \foreach \y in {0,...,3} {
        \pgfmathsetmacro{\midx}{\x+.5}
        \pgfmathsetmacro{\midy}{\y+.5}
        \coordinate (bulk-pl-\x-\y) at (\midx,\midy);
      }
    }
  \end{scope}
}

\NewDocumentCommand{\drawscinneredges}{m m m}{%
  \setcounter{edgecounter}{0}
  \foreach \x [parse=true] in {0,...,#1 - 1} {
    \pgfmathtruncatemacro{\xp}{\x+1}
    \foreach \y in {0,...,#2} {
      \drawsubedge[psc-edge]{(#3-\x-\y.east) -- (#3-\xp-\y.west)}
    }
  }
  \foreach \y [parse=true] in {0,...,#2 - 1} {
    \pgfmathtruncatemacro{\yp}{\y+1}
    \foreach \x in {0,...,#1} {
      \drawsubedge[psc-edge]{(#3-\x-\y.north) -- (#3-\x-\yp.south)}
    }
  }
}

\NewDocumentCommand{\drawscouteredges}{m m m}{%
  \foreach \x [parse=true] in {0,...,#1-1} {
    \pgfmathtruncatemacro{\xpo}{\x+1}
    \ifodd\x
      \ifodd#2\relax\else
        \drawsubedge[psc-edge]{(#3-\x-#2.north) to[bend left] (#3-\xpo-#2.north)}
      \fi
    \else
      \drawsubedge[psc-edge]{(#3-\x-0.south) to[bend right] (#3-\xpo-0.south)}
      \ifodd#2
        \drawsubedge[psc-edge]{(#3-\x-#2.north) to[bend left] (#3-\xpo-#2.north)}
      \fi
    \fi
  }
  \foreach \y [parse=true] in {0,...,#2-1} {
    \pgfmathtruncatemacro{\ypo}{\y+1}
    \ifodd\y
      \drawsubedge[psc-edge]{(#3-0-\y.west) to[bend left] (#3-0-\ypo.west)}
      \ifodd#1
        \drawsubedge[psc-edge]{(#3-#1-\y.east) to[bend right] (#3-#1-\ypo.east)}
      \fi
    \else
      \ifodd#1\relax\else
        \drawsubedge[psc-edge]{(#3-#1-\y.east) to[bend right] (#3-#1-\ypo.east)}
      \fi
    \fi
  }
}

\NewDocumentCommand{\drawscedges}{m}{%
  \begin{scope}[
    % psc-edge/.append style={edge counter label},
    ]
    \setcounter{edgecounter}{0}
    \foreach \x in {0,...,3} {
      \pgfmathtruncatemacro{\xp}{\x+1}
      \foreach \y in {0,...,4} {
        \drawsubedge[psc-edge]{(#1-\x-\y.east) -- (#1-\xp-\y.west)}
      }
    }
    \foreach \x in {0,2} {
      \pgfmathtruncatemacro{\xp}{\x+1}
      \drawsubedge[psc-edge]{(#1-\x-0.south) to[bend right] (#1-\xp-0.south)}
    }
    \foreach \x in {1,3} {
      \pgfmathtruncatemacro{\xp}{\x+1}
      \drawsubedge[psc-edge]{(#1-\xp-4.north) to[bend right] (#1-\x-4.north)}
    }
    \foreach \y in {1,3} {
      \pgfmathtruncatemacro{\yp}{\y+1}
      \drawsubedge[psc-edge]{(#1-0-\yp.west) to[bend right] (#1-0-\y.west)}
    }
    \foreach \y in {0,2} {
      \pgfmathtruncatemacro{\yp}{\y+1}
      \drawsubedge[psc-edge]{(#1-4-\y.east) to[bend right] (#1-4-\yp.east)}
    }
    \foreach \y in {0,...,3} {
      \pgfmathtruncatemacro{\yp}{\y+1}
      \foreach \x in {0,...,4} {
        \drawsubedge[psc-edge]{(#1-\x-\y.north) -- (#1-\x-\yp.south)}
      }
    }
  \end{scope}
}
\newcommand{\lbldmndop}[2]{
  \ifcase#2\relax
    \def\cda{east}
    \def\cdb{north}
    \def\pauliop{X}
  \or
    \def\cda{north}
    \def\cdb{west}
    \def\pauliop{Z}
  \or
    \def\cda{west}
    \def\cdb{south}
    \def\pauliop{X}
  \or
    \def\cda{south}
    \def\cdb{east}
    \def\pauliop{Z}
  \fi
  \path (#1.\cda) -- node[midway,sloped,pauli bg] {\(\pauliop\)} (#1.\cdb);
}


==> figures/preamble.tex <==
\usepackage{lib/mjsketch}


